DecompX: Explaining Transformers Decisions by Propagating Token Decomposition

An emerging solution for explaining Transformer-based models is to use vector-based analysis on how the representations are formed. However, providing a faithful vector-based explanation for a multi-layer model could be challenging in three aspects: (1) Incorporating all components into the analysis, (2) Aggregating the layer dynamics to determine the information flow and mixture throughout the entire model, and (3) Identifying the connection between the vector-based analysis and the model's predictions. In this paper, we present DecompX to tackle these challenges. DecompX is based on the construction of decomposed token representations and their successive propagation throughout the model without mixing them in between layers. Additionally, our proposal provides multiple advantages over existing solutions for its inclusion of all encoder components (especially nonlinear feed-forward networks) and the classification head. The former allows acquiring precise vectors while the latter transforms the decomposition into meaningful prediction-based values, eliminating the need for norm- or summation-based vector aggregation. According to the standard faithfulness evaluations, DecompX consistently outperforms existing gradient-based and vector-based approaches on various datasets. Our code is available at https://github.com/mohsenfayyaz/DecompX.

==> figs/decomposition_cls_diagram.tex <==
\begin{figure}[t]
\centering
    % left bottom right top
    \includegraphics[width=0.49\textwidth, trim=0 0 300 0, clip]{./figs/files/decomposition_cls_diagram.pdf}
    \caption{The structure of our explainability method. Our method propagates the decomposed token representations and prevents mixing them between layers. Additionally, We pass the decomposed vectors through the classification head, acquiring the exact positive/negative effect of each input token on individual labels.
    }
    \label{fig:decomposition_cls_diagram}
\end{figure}

==> figs/decomposition_globenc_diagram.tex <==
\begin{figure}[t]
\centering
    % left bottom right top
    \includegraphics[width=0.48\textwidth, trim=0 60 180 0, clip]{./figs/files/decomposition_globenc_diagram.pdf}
    \caption{The structure of our method and GlobEnc. Our method propagates the decomposed token representations and prevents mixing them between layers.
    }
    \label{fig:decomposition_globenc_diagram}
\end{figure}

==> tables/ablation_min.tex <==
\begin{table}[t!]
\begin{center}
\small
% \small
\tabcolsep=0.13cm
\begin{tabular}{l c c | c c | c c | c c} 
 \toprule
    %   & \multicolumn{4}{c}{\textbf{Attention Rollout}} \\
    % \cmidrule(lr){2-4}
     & 
     \multicolumn{2}{c}{\textbf{\textsc{SST2}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{MNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{QNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{HateXplain}}} \\
     \cmidrule(lr){2-9}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}} \\
    % \textbf{Task} & F1 Score & Compression & F1 Score & Compression & F1 Score & Compression \\
    \midrule
    DecompX
        & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \quad - Bias
        & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \quad - FFN 
        & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \quad - Cls. Head
        & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 \bottomrule
\end{tabular}
\end{center}
\captionsetup{aboveskip=0pt}
\caption{
...
}
\label{tab:ablation_table}
\end{table}


==> tables/ablation_min_full.tex <==
\begin{table*}[t!]
\begin{center}
% \small
\tabcolsep=0.13cm
\begin{tabular}{l c c | c c | c c | c c} 
 \toprule
    %   & \multicolumn{4}{c}{\textbf{Attention Rollout}} \\
    % \cmidrule(lr){2-4}
     & 
     \multicolumn{2}{c}{\textbf{\textsc{SST2}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{MNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{QNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{HateXplain}}} \\
     \cmidrule(lr){2-9}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}} \\
    % \textbf{Task} & F1 Score & Compression & F1 Score & Compression & F1 Score & Compression \\
    \midrule
    DecompX
&\underline{0.024}&\underline{92.06}& \textbf{0.129}  &\underline{76.69}&\textbf{0.093}   & \textbf{85.26}   & \underline{0.145}& \textbf{65.71} \\
    \quad w/o Bias
& \textbf{0.022}  &\textbf{92.33}   &\underline{0.141}& 75.77           &\underline{0.110}& 84.12            & \textbf{0.143}   & \underline{65.50} \\
    \quad w/o FFN 
& 0.041           & 90.95           & 0.231           & 69.20           & 0.153           & 80.65            & 0.199            & 61.73 \\
    \quad w/o Classification Head
& 0.081           & 88.23           & 0.150           &\textbf{76.77}   & 0.111           & \underline{85.19}& 0.211            & 63.08 \\
 \bottomrule
\end{tabular}
\end{center}
\captionsetup{aboveskip=0pt}
\caption{
Complete results of our ablation study when masking the \emph{least} important tokens. We employ Leave-on out ablation analysis to demonstrate bias, FFN, and classification head effects on the faithfulness of our method. The \textbf{best} and \underline{second best} results are shown by being bold and underlined respectively.
}
\label{tab:ablation_table_full}
\end{table*}


==> tables/bias_min_full.tex <==
\begin{table*}[t!]
\begin{center}
% \small
\tabcolsep=0.13cm
\begin{tabular}{l c c | c c | c c | c c} 
 \toprule
    %   & \multicolumn{4}{c}{\textbf{Attention Rollout}} \\
    % \cmidrule(lr){2-4}
     & 
     \multicolumn{2}{c}{\textbf{\textsc{SST2}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{MNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{QNLI}}} & 
     \multicolumn{2}{c}{\textbf{\textsc{HateXplain}}} \\
     \cmidrule(lr){2-9}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}}
     & \scriptsize{\textbf{\textsc{AOPC$^+$$\downarrow$}}} & \scriptsize{\textbf{\textsc{Acc$\uparrow$}}} \\
    % \textbf{Task} & F1 Score & Compression & F1 Score & Compression & F1 Score & Compression \\
    \midrule
    DecompX AbsDot Bias
&           0.024 &           92.06 &   \textbf{0.129}&   \textbf{76.69}&   \textbf{0.093}&   \textbf{85.26}&           0.145 &   \textbf{65.71} \\
    DecompX AbsSim Bias
&   \textbf{0.022}&   \textbf{92.43}&           0.138 &           75.95 &           0.106 &           84.47 &\underline{0.144}&\underline{65.57} \\
    DecompX Norm Bias 
&\underline{0.023}&           92.27 &\underline{0.132}&\underline{76.49}&\underline{0.100}&\underline{84.84}&\underline{0.144}&           65.38 \\
    DecompX Equal Bias
&   \textbf{0.022}&\underline{92.33}&           0.141 &           75.77 &           0.110 &           84.12 &   \textbf{0.143}&           65.50 \\
    DecompX No Bias
&   \textbf{0.022}&\underline{92.33}&           0.141 &           75.77 &           0.110 &           84.12 &   \textbf{0.143}&           65.50 \\
 \bottomrule
\end{tabular}
\end{center}
\captionsetup{aboveskip=0pt}
\caption{
Complete results of our bias study when masking the \emph{least} important tokens.
}
\label{tab:bias_table_full}
\end{table*}

